CN2F: A Cloud-Native Cellular Network Framework

Upcoming cellular networks aim to improve the efficiency and flexibility of mobile networks by incorporating various technologies, such as Software-Defined Networking (SDN), Network Function Virtualization (NFV), and Network Slicing (NS). There exist open-source projects that implement components of different cellular generations. In this paper, we elaborate on how to use these open-source projects to realize a flexible and extendable testbed for conducting experiments on the future generation of cellular networks. In particular, a Cloud-Native Cellular Network Framework (CN2F) is presented, which uses OpenAirInterface's codebase to generate cellular Virtual Network Functions (VNFs) and deploys Kubernetes to disperse and manage them among multiple worker nodes. Moreover, CN2F leverages ONOS and Mininet to emulate the effect of the IP transport networks in the fronthaul and backhaul of real-world cellular networks. Using CN2F, we implement different network scenarios, including Edge Computing (EC), Cloud Computing (CC), and Radio Access Network (RAN) slicing, to showcase the effectiveness of the proposed testbed for academia and industrial Research and Development (R&D) activities.

==> figs/authors.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Sepehr.png}}]{Sepehr Ganji}
received the BSc degree in computer engineering from Isfahan University of Technology, Iran, in 2023. He is currently working toward the MSc degree in the Department of Computer Science, University of Calgary, Canada. His research interests include cloud computing, networking, and multimedia. He worked as an undergraduate research assistant in the Intelligent Mobile Networks (ION) laboratory in Isfahan University of Technology from September 2021 to June 2023.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Shirin.png}}]{Shirin Behnaminia}
is currently working toward the BSc degree in the Department of Electrical and Computer Engineering, Isfahan University of Technology, Iran. Her research interests include cloud computing, networking, and distributed systems. She has worked as an undergraduate research assistant in the Intelligent Mobile Networks (ION) laboratory in Isfahan University of Technology since June 2022.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Ali.png}}]{Ali Ahangarpour}
received the BSc degree in computer engineering from Isfahan University of Technology, Iran, in 2023. He is currently working toward the MSc degree in the Department of Computer Science, University of Victoria, Canada. His research interests include cellular networks, IoT, and multimedia. He worked as an undergraduate research assistant in the Intelligent Mobile Networks (ION) laboratory in Isfahan University of Technology from June 2022 to July 2023.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Erfan2.png}}]{Erfan Mazaheri}
received the BSc degree in computer engineering from Isfahan University of Technology, Iran, in 2022, where he is currently working toward the MSc degree. His research interests include machine learning, distributed systems, and IoT. He worked as an undergraduate research assistant in the Intelligent Mobile Networks (ION) laboratory in Isfahan University of Technology from February 2022 to July 2023.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Sara.png}}]{Sara Baradaran}
received the BSc degree in computer engineering from Isfahan University of Technology, Iran, in 2022. She is currently working toward the PhD degree in the Department of Computer Science, University of Southern California, USA. Her research interests include software engineering, program analysis, and software verification. She worked as an undergraduate research assistant in the Intelligent Mobile Networks (ION) laboratory in Isfahan University of Technology from November 2022 to February 2023.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Zeinab.png}}]{Zeinab Zali}
received the BSc degree in software engineering and the MSc degree in Artificial Intelligent from Isfahan University of Technology, Iran, in 2006 and 2009, respectively. She received the PhD degree in computer engineering from Isfahan University of Technology in 2017. She was also a visiting student with the Telematic Laboratory, Politecnico de Bari, in 2014. She is currently an assistant professor in the Department of Electrical and Computer Engineering at Isfahan University of Technology. Her research interests include operating systems, distributed systems, IoT, Fog and cloud computing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/MohammadReza.png}}]{Mohammad Reza Heidarpour}
received the BSc and MSc degrees in electronics and communication engineering from Isfahan University of Technology, Iran, in 2006 and 2008, respectively, and the PhD degree in electrical engineering from the University of Waterloo, Canada, in 2013. He has done post-doctoral research at the Coding and Signal Transmission (CST) laboratory in the University of Waterloo from May 2013 to November 2015 and at Isfahan University of Technology from December 2016 to October 2017. He is currently an assistant professor in the Department of Electrical and Computer Engineering at Isfahan University of Technology. His research interests include broad areas of wireless communication, data networks, and network algorithms.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Rakhshan.png}}]{Ali Rakhshan}
received the graduate degrees from the University of Massachusetts Amherst, USA. He has worked as a post-doctoral research fellow and assistant research scientist at the Johns Hopkins University, USA. He is currently a research scientist at Mobile Communications Company of Iran (MCI). In addition to academic positions and publishing several papers, he has also work experience in the USA industry. He has also contributed to a notable textbook on probability and statistics.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Faraji.png}}]{Mahsa Faraji Shoyari}
received the MSc degree in computer engineering from Sharif University of Technology, Iran, in 2018. She is currently a senior cloud engineer at the R\&D Department of the Mobile Communications Company of Iran (MCI). Her main research interests include cloud computing, performance/dependability modeling and evaluation, distributed computing systems, and resource scheduling algorithms.
\end{IEEEbiography}
